Analytic Class Incremental Learning for Sound Source Localization with Privacy Protection

Sound Source Localization (SSL) enabling technology for applications such as surveillance and robotics. While traditional Signal Processing (SP)-based SSL methods provide analytic solutions under specific signal and noise assumptions, recent Deep Learning (DL)-based methods have significantly outperformed them. However, their success depends on extensive training data and substantial computational resources. Moreover, they often rely on large-scale annotated spatial data and may struggle when adapting to evolving sound classes. To mitigate these challenges, we propose a novel Class Incremental Learning (CIL) approach, termed SSL-CIL, which avoids serious accuracy degradation due to catastrophic forgetting by incrementally updating the DL-based SSL model through a closed-form analytic solution. In particular, data privacy is ensured since the learning process does not revisit any historical data (exemplar-free), which is more suitable for smart home scenarios. Empirical results in the public SSLR dataset demonstrate the superior performance of our proposal, achieving a localization accuracy of 90.9%, surpassing other competitive methods.

==> response1.tex <==
\begin{document}
\section*{SPL-32693-2022: Response Letter}

Dear Dr Tsao Yu, \\

We are truly grateful to yours and other reviewers' {valuable} comments and thoughtful suggestions on our manuscript. According to these comments and suggestions, we have made careful modifications to the original manuscript.
Please find enclosed the revised manuscript ``Deep Audio-visual Beamforming for Speaker Localizatio''​ (SPL-32693-2022). In this letter, we numbered the comments of each reviewer and provided our detailed response. The reviewers' comments are in black color. The authors’ reply and the description of the changes we have implemented are in blue color. To facilitate the review, we uploaded a version of the revised manuscript that highlights the main changes with respect to the previous version.\\

We hope that these revisions are satisfactory and that the revised version will be acceptable for publication in IEEE Signal Processing Letters.\\

Yours sincerely,

\vspace{1cm}

\noindent
Xinyuan Qian\\
Qiquan Zhang\\
Guohui Guan\\
Wei Xue

\end{document}
